Over then Under Tangles

Over-then-Under (OU) tangles are oriented tangles whose strands travel through all of their over crossings before any under crossings. In this paper we discuss the idea of gliding: an algorithm by which any tangle diagram could be brought to OU form. Unfortunately, the algorithm is flawed. However, by analyzing cases in which it does succeed we obtain a braid classification result, which we also extend to virtual braids, and provide a Mathematica implementation. We discuss other instances of successful "gliding ideas" which appear in the literature - sometimes in disguise - such as the Drinfel'd double construction, Enriquez's work on quantization of Lie bialgebras, and Audoux and Meilhan's classification of welded homotopy links,

==> t.tex <==
\section{Theorems and Proofs}\label{sec:Theorems}

As we shall see in this section, everything in the previous section holds
true for braids, and hence we get a nice OU theorem for braids, ``every
braid, when considered as a tangle, has a unique reduced OU form'', so
braids can be be separated by their OU forms. As we shall also see here,
everything in the previous section extends to virtual tangles, and is true
when restricted to virtual braids. Thus we find that every virtual braid
has a unique OU form when it is regarded as a virtual tangle; with extra
work we find that this OU form is a complete invariant of virtual braids.

\draftcut \input c.tex

\draftcut \input v.tex

\draftcut \input a.tex

